1-bit Adam: Communication Efficient Large-Scale Training with Adam's Convergence Speed

Scalable training of large models (like BERT and GPT-3) requires careful optimization rooted in model design, architecture, and system capabilities. From a system standpoint, communication has become a major bottleneck, especially on commodity systems with standard TCP interconnects that offer limited network bandwidth. Communication compression is an important technique to reduce training time on such systems. One of the most effective methods is error-compensated compression, which offers robust convergence speed even under 1-bit compression. However, state-of-the-art error compensation techniques only work with basic optimizers like SGD and momentum SGD, which are linearly dependent on the gradients. They do not work with non-linear gradient-based optimizers like Adam, which offer state-of-the-art convergence efficiency and accuracy for models like BERT. In this paper, we propose 1-bit Adam that reduces the communication volume by up to $5\times$, offers much better scalability, and provides the same convergence speed as uncompressed Adam. Our key finding is that Adam's variance (non-linear term) becomes stable (after a warmup phase) and can be used as a fixed precondition for the rest of the training (compression phase). Experiments on up to 256 GPUs show that 1-bit Adam enables up to $3.3\times$ higher throughput for BERT-Large pre-training and up to $2.9\times$ higher throughput for SQuAD fine-tuning. In addition, we provide theoretical analysis for our proposed work.

==> asyn.tex <==
\newpage

\begin{center}
    \LARGE{ Supplementary Material}
\end{center}

We provide the proofs to our theorems in the supplemental material.

\section*{Preliminaries} Below we would use some basic properties of matrix and vector.
\begin{itemize}
\item For any $A\in \mathbb R^{d\times n} $ and $P \in \mathbb R^{n\times n} $, if $PP^{\top}  = I$, then we have
\begin{align*}
\|AP\|_F^2 = \|AP^{\top}\|_F^2 = \|A\|_F^2.
\end{align*}
\item For any two vectors $\bm{a} $ and $\bm{b}$, we have
\begin{align*}
\|\bm{a} + \bm{b} \|^2 \leq (1 + \alpha)\|\bm{a}\|^2 + \left( 1 + \frac{1}{\alpha} \right)\|\bm{b}\|^2, \quad\forall \alpha > 0.
\end{align*}
\item For any two matrices $A $ and $B$, we have
\begin{align*}
\|A + B \|^2_F \leq (1 + \alpha)\|A\|^2_F + \left( 1 + \frac{1}{\alpha} \right)\|B\|^2_F, \quad\forall \alpha > 0.
\end{align*}
\end{itemize}

Before presenting our proof, we first rewrite our updating rule  as follows
\begin{align*}
\Delta_t =& (X_t - \gamma G_t) + \Delta_{t-1} - C_{\omega}\left[ (X_t - \gamma G_t) + \Delta_{t-1} \right]\\
X_{t+1} =& (X_t - \gamma G_t) W_{\eff}+ \eta (\Delta_{t-1} - \Delta_t) (W_{\eff}-I) \numberthis\label{general:updating_rule}
\end{align*}
where 
\begin{align*}
W_{\eff} := (1-\eta)I + \eta W.
\end{align*}


\section*{Proof of Lemma~\ref{lemma:key_theo_lemma}} \label{sec:proof_key_lemma}

Lemma \ref{lemma:key_theo_lemma} is the key lemma for proving our Theorem \ref{theo}. 

\begin{lemma}\label{lemma:key_theo_lemma}
For  algorithm that admits the updating rule \eqref{general:updating_rule}, if 
\begin{align*}
W_{\eff} \succeq & 0,\\
(2 - \lambda_n )^2(3 - 2\lambda_n) \leq & \frac{1}{\alpha^2},\\
 1 -3C_5L^2\gamma^2 \geq & 0,\\
 L \leq & \frac{1}{L}
\end{align*}
then we have
\begin{align*}
&\left(\frac{\gamma}{2} -\frac{3C_5L^2 \gamma^3}{2 -6C_5L^2\gamma^2} \right)\sum_{t=0}^T E \left\|\nabla f(\overline{\bm{x}}_t)\right\|^2\\
\leq & \mathbb E f\left(\overline{\bm{x}}_{0} \right) - \mathbb E f\left(\bm{x}^* \right)  + \left(\frac{L\gamma^2}{2} + \frac{C_5L^2\gamma^3}{2 -6C_5L^2\gamma^2)}\right)\sigma^2T + \frac{3C_5L^2\gamma^3\zeta^2T}{2 -6C_5L^2\gamma^2}.
\end{align*}
where 
\begin{align*}
C_4 := & \frac{\alpha^2}{(1 - \alpha^2(2-\lambda_n)^2(3 -2\lambda_n) )(1-\lambda_n)^2} \\
 C_5 := & \frac{3}{(1-\lambda_2)^2} + 6C_4,
\end{align*}
and $\lambda_n = \lambda_n(W_{\eff})$ and $\lambda_2 = \lambda_2(W_{\eff})$ for short.
\end{lemma}

We outline our proof of Lemma \ref{lemma:key_theo_lemma} as follows.

The most challenging part of a decentralized algorithm, unlike the centralized algorithm, is that we need to ensure the local model on each node to converge to the average value $\overline{\bm{x}}_t$. This is because
\begin{align*}
&\mathbb E f\left(\overline{\bm{x}}_{t+1} \right) - \mathbb E f\left(\overline{\bm{x}}_{t} \right)\\
\leq & -\frac{\gamma}{2}\mathbb E \left\|\nabla \of(X_t)\right\|^2 -\left(\frac{\gamma}{2} -\frac{L\gamma^2}{2}\right) \mathbb E \left\|\nabla \of(X_t)\right\|^2 + \frac{\gamma L^2}{2n}\mathbb E \left\|X_t(I - A_n) \right\|^2_F+ \frac{L\gamma^2\sigma^2}{2n}.\numberthis\label{lemma:why_bound_diff}
\end{align*}

So  we first prove that
\begin{align*}
\sum_{t=0}^{T-1}\sum_{i=1}^n \left\|\overline{\bm{x}}_t - \bm{x}_t^{(i)} \right\|^2 = &  \sum_{t=0}^{T-1} \mathbb E\left\|X_t(I - A_n)\right\|_F^2\\
\leq & \frac{3\gamma^2}{(1-\lambda_2)^2}\sum_{t=0}^{T-2}\left\|G_t\right\|^2_F + 6\sum_{t=0}^{T-1} \left\|\Delta_{t}(W_{\eff}-I) \right\|_F^2,
\end{align*}
and the compressing error can be upper bounded by
\begin{align*}
\sum_{t=0}^{T-1}\mathbb E\left\|\Delta_{t}(W_{\eff}-I)\right\|^2 \leq C_4\gamma^2\sum_{t=0}^{T-1} \mathbb E\left\|G_t \right\|^2_F.
\end{align*}
With these two important observations, we finally prove that
\begin{align*}
\sum_{t=0}^{T-1} \mathbb E\left\|X_t(I - A_n)\right\|_F^2 \leq \frac{C_5\gamma^2n\sigma^2 T}{1 -3C_5L^2\gamma^2} + \frac{3nC_5\gamma^2\zeta^2 T}{1 -3C_5L^2\gamma^2} + \sum_{t=0}^{T-1}\frac{3nC_5 \gamma^2\mathbb{E}\left\|\nabla f(\overline{\bm{x}}_t)\right\|^2}{1 -3C_5L^2\gamma^2}.
\end{align*}
So taking the equation above into \eqref{lemma:why_bound_diff} we could directly prove Theorem~\ref{lemma:key_theo_lemma}.


Now we introduce the detailed proof for Lemma \ref{lemma:key_theo_lemma}.



\paragraph{Proof of Lemma~\ref{lemma:key_theo_lemma}}
\begin{proof}
The updating rule of $\OA$ can be written as
\begin{align*}
\Delta_t =&  -\gamma G_t + X_t  + \Delta_{t - 1} - C_\omega\left[  -\gamma G_t + X_t  + \Delta_{t - 1} \right],\\
X_{t+1} =& (X_t - \gamma G_t) W_{\eff} + (\Delta_{t-1} - \Delta_t) (W_{\eff}-I),
\end{align*}

The updating rule of $\overline{\bm{x}}_t$ can be conducted using the equation above
\begin{align*}
\overline{\bm{x}}_{t+1} =& \overline{\bm{x}}_t - \gamma\bG_t.
\end{align*}
So we have
\begin{align*}
&\mathbb E f\left(\overline{\bm{x}}_{t+1} \right) - \mathbb E f\left(\overline{\bm{x}}_{t} \right)\\
\leq & - \gamma\mathbb E \left\langle \bG_t,\nabla f(\overline{\bm{x}}_t) \right\rangle + \frac{L\gamma^2}{2}\mathbb E \left\|\bG_t\right\|^2\\
= & - \gamma\mathbb E \left\langle \nabla \of(X_t),\nabla f(\overline{\bm{x}}_t) \right\rangle + \frac{L\gamma^2}{2}\mathbb E \left\|\bG_t - \nabla\of(X_t)\right\|^2 + \frac{L\gamma^2}{2}\mathbb E \left\|\nabla\of(X_t)\right\|^2\\
= & - \gamma\mathbb E \left\langle\nabla  \of(X_t),\nabla f(\overline{\bm{x}}_t) \right\rangle + \frac{L\gamma^2}{2}\mathbb E \left\|\nabla\of(X_t)\right\|^2 + \frac{L\gamma^2\sigma^2}{2n}.
\end{align*}
Using
\begin{align*}
\left\langle\nabla  \of(X_t),\nabla f(\overline{\bm{x}}_t) \right\rangle = \frac{1}{2}\left( \left\|\nabla \of(X_t)\right\|^2 + \left\|\nabla f(\overline{\bm{x}}_t)\right\|^2 - \left\|\nabla \of(X_t) -\nabla f(\overline{\bm{x}}_t)\right\|^2\right),
\end{align*}
then the equation above becomes
\begin{align*}
&\mathbb E f\left(\overline{\bm{x}}_{t+1} \right) - \mathbb E f\left(\overline{\bm{x}}_{t} \right)\\
\leq &  - \frac{\gamma}{2}\left( \mathbb E \left\|\nabla \of(X_t)\right\|^2 + \mathbb E \left\|\nabla f(\overline{\bm{x}}_t)\right\|^2 - \mathbb E \left\|\nabla \of(X_t) -\nabla f(\overline{\bm{x}}_t)\right\|^2\right) \\
&+ \frac{L\gamma^2}{2}\mathbb E \left\|\nabla\of(X_t)\right\|^2 + \frac{L\gamma^2\sigma^2}{2n}\\
= & -\frac{\gamma}{2}\mathbb E \left\|\nabla f(\overline{\bm{x}}_t)\right\|^2 -\left(\frac{\gamma}{2} -\frac{L\gamma^2}{2}\right) \mathbb E \left\|\nabla \of(X_t)\right\|^2 + \frac{\gamma}{2}\mathbb E \left\|\nabla \of(X_t) -\nabla f(\overline{\bm{x}}_t)\right\|^2+ \frac{L\gamma^2\sigma^2}{2n}.\numberthis\label{supp:theo_eq1}
\end{align*}
The difference between $\nabla \of(X_t) $ and $\nabla f(\overline{\bm{x}}_t)$ can be upper bounded by
\begin{align*}
\mathbb E\left\|\nabla \of(X_t) -\nabla f(\overline{\bm{x}}_t)\right\|^2 = & \mathbb E\left\|\frac{1}{n}\sum_{i=1}^n \nabla f_i(\bm{x}_t^{(i)}) - \nabla f_i(\overline{\bm{x}}_t) \right\|^2\\
\leq &\frac{1}{n^2}\mathbb E\left\|\sum_{i=1}^n \nabla f_i(\bm{x}_t^{(i)}) - \nabla f_i(\overline{\bm{x}}_t) \right\|^2\\
\leq & \frac{1}{n}\sum_{i=1}^n\mathbb E\left\| \nabla f_i(\bm{x}_t^{(i)}) - \nabla f_i(\overline{\bm{x}}_t) \right\|^2\\
\leq & \frac{L^2}{n}\sum_{i=1}^n\mathbb E\left\| \bm{x}_t^{(i)} - \overline{\bm{x}}_t \right\|^2\\
= & \frac{L^2}{n}\mathbb E\left\|X_t(I - A_n) \right\|^2_F.
\end{align*}
So \eqref{supp:theo_eq1} becomes
\begin{align*}
&\mathbb E f\left(\overline{\bm{x}}_{t+1} \right) - \mathbb E f\left(\overline{\bm{x}}_{t} \right)\\
\leq & -\frac{\gamma}{2}\mathbb E \left\|\nabla f(\overline{\bm{x}}_t)\right\|^2 -\left(\frac{\gamma}{2} -\frac{L\gamma^2}{2}\right) \mathbb E \left\|\nabla \of(X_t)\right\|^2 + \frac{\gamma L^2}{2n}\mathbb E \left\|X_t(I - A_n) \right\|^2_F+ \frac{L\gamma^2\sigma^2}{2n}.
\end{align*}
Continuing using Lemma~\ref{lemma:bound_diff_X} to give upper bound for $\mathbb E \left\|X_t(I - A_n) \right\|^2_F$, we have
\begin{align*}
&\mathbb E f\left(\overline{\bm{x}}_{t+1} \right) - \mathbb E f\left(\overline{\bm{x}}_{t} \right)\\
\leq & -\frac{\gamma}{2}\mathbb E \left\|\nabla \of(X_t)\right\|^2 -\left(\frac{\gamma}{2} -\frac{L\gamma^2}{2}\right) \mathbb E \left\|\nabla \of(X_t)\right\|^2 + \frac{\gamma L^2}{2n}\mathbb E \left\|X_t(I - A_n) \right\|^2_F+ \frac{L\gamma^2\sigma^2}{2n}\\
\leq & -\frac{\gamma}{2}\mathbb E \left\|\nabla f(\overline{\bm{x}}_t)\right\|^2 -\left(\frac{\gamma}{2} -\frac{L\gamma^2}{2}\right) \mathbb E \left\|\nabla \of(X_t)\right\|^2 + \frac{L\gamma^2\sigma^2}{2n}\\
& + \frac{C_5L^2\gamma^3\sigma^2}{2 -6C_5L^2\gamma^2)} + \frac{3C_5L^2\gamma^3\zeta^2}{2 -6C_5L^2\gamma^2} + \frac{3C_5L^2 \gamma^3\mathbb{E}\left\|\nabla f(\overline{\bm{x}}_t)\right\|^2}{2 -6C_5L^2\gamma^2},
\end{align*}
which can be rewritten as
\begin{align*}
&\left(\frac{\gamma}{2} -\frac{3C_5L^2 \gamma^3}{2 -6C_5L^2\gamma^2} \right) E \left\|\nabla f(\overline{\bm{x}}_t)\right\|^2\\ \leq & \mathbb E f\left(\overline{\bm{x}}_{t} \right) - \mathbb E f\left(\overline{\bm{x}}_{t+1} \right) - \left(\frac{\gamma}{2} -\frac{L\gamma^2}{2}   \right)\mathbb{E}\left\|\nabla \of(X_t)\right\|^2 + \left(\frac{L\gamma^2}{2n} + \frac{C_5L^2\gamma^3}{2 -6C_5L^2\gamma^2)}\right)\sigma^2\\
& + \frac{3C_5L^2\gamma^3\zeta^2}{2 -6C_5L^2\gamma^2}.
\end{align*}
Summing up the equation above from $t=0$ to $t=T-1$ we get
\begin{align*}
&\left(\frac{\gamma}{2} -\frac{3C_5L^2 \gamma^3}{2 -6C_5L^2\gamma^2} \right)\sum_{t=0}^T E \left\|\nabla f(\overline{\bm{x}}_t)\right\|^2\\
\leq & \mathbb E f\left(\overline{\bm{x}}_{0} \right) - \mathbb E f\left(\overline{\bm{x}}_{T} \right)  + \left(\frac{L\gamma^2}{2n} + \frac{C_5L^2\gamma^3}{2 -6C_5L^2\gamma^2}\right)\sigma^2T+ \frac{3C_5L^2\gamma^3\zeta^2T}{2 -6C_5L^2\gamma^2}.\quad\text{($\gamma\leq \frac{1}{L}$)}
\end{align*}

This concludes the proof.
\end{proof}

Below are some critical lemmas for the proof of Lemma \ref{lemma:key_theo_lemma}. 

\begin{lemma}\label{lemma:seq}
Given two non-negative sequences $\{a_t\}_{t=1}^{\infty}$ and $\{b_t\}_{t=1}^{\infty}$ that satisfying
\begin{equation}
a_t =  \sum_{s=1}^t\rho^{t-s}b_{s}, \numberthis \label{eqn1}
\end{equation}
with $\rho\in[0,1)$, we have
\begin{align*}
D_k:=\sum_{t=1}^{k}a_t^2 \leq & % \frac{(1+\frac{2\rho}{1-\rho})\sum_{t=1}^kb_t^2-\rho^2a_k^2}{1-\rho^2} \\ \leq & 
\frac{1}{(1-\rho)^2} \sum_{s=1}^kb_s^2.
\end{align*}
%where $S_k=\sum_{t=1}^{k}a_t$, and $D_k=\sum_{t=1}^{k}a_t^2$.
\end{lemma}

\begin{proof}
From the definition, we have
\begin{align*}
S_k= & \sum_{t=1}^{k}\sum_{s=1}^t\rho^{t-s}b_{s}
=  \sum_{s=1}^{k}\sum_{t=s}^k\rho^{t-s}b_{s}
=  \sum_{s=1}^{k}\sum_{t=0}^{k-s}\rho^{t}b_{s}
\leq  \sum_{s=1}^{k}{b_{s}\over 1-\rho}, \numberthis \label{eqn3}\\
D_k=  & \sum_{t=1}^{k}\sum_{s=1}^t\rho^{t-s}b_{s}\sum_{r=1}^t\rho^{t-r}b_{r}\\
= & \sum_{t=1}^{k}\sum_{s=1}^t\sum_{r=1}^t\rho^{2t-s-r}b_{s}b_{r} \\
\leq &  \sum_{t=1}^{k}\sum_{s=1}^t\sum_{r=1}^t\rho^{2t-s-r}{b_{s}^2+b_{r}^2\over2}\\
= & \sum_{t=1}^{k}\sum_{s=1}^t\sum_{r=1}^t\rho^{2t-s-r}b_{s}^2 \\
\leq  & {1\over 1-\rho}\sum_{t=1}^{k}\sum_{s=1}^t\rho^{t-s}b_{s}^2\\
\leq & {1\over (1-\rho)^2}\sum_{s=1}^{k}b_{s}^2. \quad \text{(due to \eqref{eqn3})}
\end{align*}
\end{proof}




\begin{lemma}\label{lemma:bound_pow2}
For any matrix sequence $\{M_t\}$ and positive integer constant $m\in\{1,2,\cdots\}$, we have
\begin{align*}
\sum_{t=0}^{T-1}\left\| \sum_{s=0}^t M_s(W_{\eff} - I)^mW_{\eff}^{t-s} \right\|^2_F \leq  (1- \lambda_n)^{2m-2}\sum_{t=0}^{T-1}\left\|  M_t \right\|^2_F.
\end{align*}
\end{lemma}


\begin{proof}
Since $W_{\eff}$ is symmetric, so we decompose it as $W_{\eff} = P\Lambda P^{\top} $.  Denote $B_s:= M_s P^{\top}$ and $\bm{b}_s^{(i)}$ be the $i$th column of $B_s$, we have
\begin{align*}
\left\| \sum_{s=0}^t M_s(W_{\eff} - I)^mW_{\eff}^{t-s} \right\|^2_F = &
\left\| \sum_{s=0}^t M_sP^{\top}(\Lambda - I)^m\Lambda^{t-s}P \right\|^2_F\\
= & \left\| \sum_{s=0}^t M_sP^{\top}(\Lambda - I)^m\Lambda^{t-s} \right\|^2_F\\
= & \left\| \sum_{s=0}^t B_s(\Lambda - I)^m\Lambda^{t-s} \right\|^2_F\\
= & \sum_{i=1}^n \left\| \sum_{s=0}^t \bm{b}_s^{(i)}(\lambda_i - 1)^m\lambda^{t-s}_i \right\|^2\\
= & \sum_{i=1}^n (\lambda_i - 1)^{2m} \left\| \sum_{s=0}^t \bm{b}_s^{(i)}\lambda^{t-s}_i \right\|^2.
\end{align*}
So we have
\begin{align*}
&\sum_{t=0}^{T-1}\left\| \sum_{s=0}^t M_s(W_{\eff} - I)^mW_{\eff}^{t-s} \right\|^2_F\\
= & \sum_{t=0}^{T-1}\sum_{i=1}^n (\lambda_i - 1)^{2m} \left\| \sum_{s=0}^t \bm{b}_s^{(i)}\lambda^{t-s}_i \right\|^2\\
= & \sum_{i=1}^n (\lambda_i - 1)^{2m} \sum_{t=0}^{T-1}\left\| \sum_{s=0}^t \bm{b}_s^{(i)}\lambda^{t-s}_i \right\|^2\\
\leq & \sum_{i=1}^n (\lambda_i - 1)^{2m} \left( \frac{1}{\left(1-\lambda_i \right)^2} \sum_{t=0}^{T-1}\left\|  \bm{b}_t^{(i)} \right\|^2 \right)\quad\text{(using Lemma~\ref{lemma:seq})} \\
= & \sum_{i=1}^n \frac{(\lambda_i - 1)^{2m}}{\left(1-\lambda_i \right)^2} \sum_{t=0}^{T-1}\left\|  \bm{b}_t^{(i)} \right\|^2 \\
\leq & (1- \lambda_n)^{2m-2}\sum_{t=0}^{T-1}\sum_{i=1}^n\left\|  \bm{b}_t^{(i)} \right\|^2\\
= & (1- \lambda_n)^{2m-2}\sum_{t=0}^{T-1}\left\|  M_t \right\|^2_F.
\end{align*}

\end{proof}





\begin{lemma}\label{lemma:bound_compress_error}
For AlgXX, we have the following upper bound for $\mathbb E\|\Delta_t (W_{\eff}-I)\|^2_F$:
\begin{align*}
\sum_{t=0}^{T-1}\mathbb E\left\|\Delta_{t}(W_{\eff}-I)\right\|^2 \leq C_4\gamma^2\sum_{t=0}^{T-1} \mathbb E\left\|G_t \right\|^2_F,
\end{align*}
when
\begin{align*}
(2 - \lambda_n )^2(3 - 2\lambda_n) \leq \frac{1}{\alpha^2}.
\end{align*}

\end{lemma}

\begin{proof}
From Assumption \label{ass:global}, for $\Delta_t$, we have
\begin{align*}
&\mathbb E\|\Delta_t (W_{\eff}-I)\|^2_F\\
 \leq &\mathbb E \alpha^2 \left\| \left (X_t - \gamma G_t + \Delta_{t-1} \right)(W_{\eff}-I) \right\|^2_F\\
= & \alpha^2\mathbb E\left\|- \gamma \sum_{s=0}^{t}G_sW_{\eff}^{t-s}(W_{\eff}-I) + \sum_{s=0}^{t-2} \Delta_{s} (W_{\eff}-I)^3W_{\eff}^{t-2-s} - \Delta_{t-1}(W_{\eff}-I)^2 + \Delta_{t-1}(W_{\eff}-I) \right\|^2_F\\
\leq & \alpha^2\mathbb E\left(1 + \frac{1}{\beta_1} \right) \left\|- \gamma \sum_{s=0}^{t}G_sW_{\eff}^{t-s}(W_{\eff}-I) + \sum_{s=0}^{t-2} \Delta_{s} (W_{\eff}-I)^3W_{\eff}^{t-2-s}  \right\|^2_F\\
& + \alpha^2(1 + \beta_1) \mathbb E\left\|\Delta_{t-1}(2I - W_{\eff})(W_{\eff}-I)\right\|^2_F\\
\leq & \alpha^2 \left(1 + \frac{1}{\beta_1} \right)(1 + \beta_2 )\mathbb E\left\| \sum_{s=0}^{t-2} \Delta_{s} (W_{\eff}-I)^3W_{\eff}^{t-2-s}  \right\|^2_F\\
& + \alpha^2\left(1 + \frac{1}{\beta_1} \right)\left(1 + \frac{1}{\beta_2} \right)\mathbb E\left\|- \gamma \sum_{s=0}^{t}G_sW_{\eff}^{t-s}(W_{\eff}-I)   \right\|^2_F\\
& + \alpha^2(1 + \beta_1)( 2 - \lambda_n )^2\mathbb E\left\|\Delta_{t-1}(W_{\eff}-I)\right\|^2.\numberthis\label{supp:key_eq1}
\end{align*}
Defining $\Delta_{-1} = \Delta_{-2} = 0$, and
bound $\left\| \sum_{s=0}^{t-2} \Delta_{s} (W_{\eff}-I)^3W_{\eff}^{t-2-s}  \right\|^2_F$ in the equation above using Lemma~\ref{lemma:bound_pow2}, which leads to
\begin{align*}
\sum_{t=0}^{T-1}\left\| \sum_{s=-2}^{t-2} \Delta_{s} (W_{\eff}-I)^3W_{\eff}^{t-2-s}  \right\|^2_F = & \sum_{t=-2}^{T-3}\left\| \sum_{s=-2}^{t} \Delta_{s} (W_{\eff}-I)^3W_{\eff}^{t-s}  \right\|^2_F \\
= & \sum_{t=0}^{T-3}\left\| \sum_{s=0}^{t} \Delta_{s} (W_{\eff}-I)^3W_{\eff}^{t-s}  \right\|^2_F\quad\text{($\Delta_{-1} = \Delta_{-2} = 0$)}\\
\leq & (1-\lambda_n )^2\sum_{t=0}^{T-3}\left\|  \Delta_{t} (W_{\eff}-I)  \right\|^2_F. \numberthis\label{supp:key_eq2}
\end{align*}
Setting $ \beta_1 = \beta_2 =  1-\lambda_n $, summing up both sides of equation \eqref{supp:key_eq1} from $t=0$ to $t=T-1$ we get
\begin{align*}
& \sum_{t=0}^{T-1} \mathbb E\|\Delta_t (W_{\eff}-I)\|^2_F\\
\leq & \alpha^2\left(  1 + \frac{1}{1-\lambda_n} \right )(2 - \lambda_n)\sum_{t=0}^{T-1}\mathbb E\left\| \sum_{s=0}^{t-2} \Delta_{t} (W_{\eff}-I)^3W_{\eff}^{t-2-s}  \right\|^2_F \\
&+ \alpha^2(2 - \lambda_n)^3\sum_{t=0}^{T-1}\mathbb E\left\|\Delta_{t-1}(W_{\eff}-I)\right\|^2\\
& + \alpha^2\left(1 + \frac{1}{1 - \lambda_n} \right )^2 \sum_{t=0}^{T-1} \mathbb E\left\|- \gamma \sum_{s=0}^{t}G_sW_{\eff}^{t-s}(W_{\eff}-I)   \right\|^2_F\\
\leq & \alpha^2\left( 2 - \lambda_n \right)^2( 1- \lambda_n) \sum_{t=0}^{T-3}\mathbb E\left\|  \Delta_{t} (W_{\eff}-I)  \right\|^2_F+ \alpha^2(2 - \lambda_n)^3\sum_{t=0}^{T-1}\mathbb E\left\|\Delta_{t-1}(W_{\eff}-I)\right\|^2\\
& + \alpha^2 \left(1 + \frac{1}{1 - \lambda_n} \right )^2 \sum_{t=0}^{T-1} \mathbb E\left\|- \gamma \sum_{s=0}^{t}G_sW_{\eff}^{t-s}(W_{\eff}-I)   \right\|^2_F\\
\leq & \alpha^2(2 -\lambda_n )^2(3 - 2\lambda_n )\sum_{t=0}^{T-1}\mathbb E\left\|\Delta_{t}(W_{\eff}-I)\right\|^2 + \frac{\alpha^2\lambda_n^2\gamma^2}{(1-\lambda_n)^2}\sum_{t=0}^{T-1} \mathbb E\left\|\sum_{s=0}^{t}G_sW_{\eff}^{t-s}(W_{\eff}-I)   \right\|^2_F\\
\leq & \alpha^2(2 -\lambda_n )^2(3 - 2\lambda_n )\sum_{t=0}^{T-1}\mathbb E\left\|\Delta_{t}(W_{\eff}-I)\right\|^2 + \frac{\alpha^2\lambda_n^2\gamma^2}{(1-\lambda_n)^2}\sum_{t=0}^{T-1} \mathbb E\left\|G_t \right\|^2_F. \quad\text{(by Lemma~\ref{lemma:bound_pow2} )}
\end{align*}
the equation above can also be written as
\begin{align*}
\left( 1 - \alpha^2(2 -\lambda_n )^2(3 - 2\lambda_n ) \right)\sum_{t=0}^{T-1}\mathbb E\left\|\Delta_{t}(W_{\eff}-I)\right\|^2 \leq \frac{\alpha^2\lambda_n^2\gamma^2}{(1-\lambda_n)^2}\sum_{t=0}^{T-1} \mathbb E\left\|G_t \right\|^2_F.
\end{align*}
So if 
\begin{align*}
&1 - \alpha^2(2 - \lambda_n )^2(3 - 2\lambda_n) \geq 0\\
&(2 - \lambda_n )^2(3 - 2\lambda_n) \leq \frac{1}{\alpha^2}
\end{align*}
then we have
\begin{align*}
\sum_{t=0}^{T-1}\mathbb E\left\|\Delta_{t}(W_{\eff}-I)\right\|^2 \leq C_4\sum_{t=0}^{T-1} \mathbb E\left\|G_t \right\|^2_F.
\end{align*}



\end{proof}

\begin{lemma} \label{lemma:bound_G}
Under the Assumption \ref{ass:global}, when using Algorithm~\ref{alg:de_ec}, we have
\begin{align*}
\mathbb{E}\left\|G(X_t,\xi_t)\right\|^2_F\leq &  n\sigma^2+3L^2\mathbb{E}\left\|X_t(I - A_n)\right\|^2_F+3n\zeta^2+3n\mathbb{E}\left\|\nabla f(\overline{\bm{x}}_t)\right\|^2.
\end{align*}
\end{lemma}


\begin{proof}
Notice that
\begin{align*}
\mathbb{E}\left\|G(X_t,\xi_t)\right\|^2_F
= \sum_{i=1}^{n}\mathbb{E}\left\|\nabla F_i(x_t^{(i)};\xi_t^{(i)})\right\|^2.
\end{align*}
We next estimate the upper bound of $\mathbb{E}\left\|\nabla F_i(\bm{x}_t^{(i)};\xi_t^{(i)})\right\|^2$ in the following
\begin{align*}
\mathbb{E}\left\|\nabla F_i(\bm{x}_t^{(i)};\xi_t^{(i)})\right\|^2
= & \mathbb{E}\left\|\left(\nabla F_i(\bm{x}_t^{(i)};\xi_t^{(i)})-\nabla f_i(\bm{x}_t^{(i)})\right)+\nabla f_i(\bm{x}_t^{(i)})\right\|^2\\
= & \mathbb{E}\left\|\nabla F_i(\bm{x}_t^{(i)};\xi_t^{(i)})-\nabla f_i(\bm{x}_t^{(i)})\right\|^2+\mathbb{E}\left\|\nabla f_i(\bm{x}_t^{(i)})\right\|^2\\
 & + 2\mathbb{E}\left\langle\mathbb{E}_{\xi_t}\nabla F_i(\bm{x}_t^{(i)};\xi_t^{(i)})-\nabla f_i(\bm{x}_t^{(i)}),\nabla f_i(\bm{x}_t^{(i)})\right\rangle\\
= &\mathbb{E}\left\|\nabla F_i(\bm{x}_t^{(i)};\xi_t^{(i)})-\nabla f_i(\bm{x}_t^{(i)})\right\|^2+\mathbb{E}\left\|\nabla f_i(\bm{x}_t^{(i)})\right\|^2\\
\leq & \sigma^2 + \mathbb{E}\left\|\left(\nabla f_i(\bm{x}_t^{(i)})-\nabla f_i(\overline{\bm{x}}_t)\right)+\left(\nabla f_i(\overline{\bm{x}}_t)-\nabla f(\overline{\bm{x}}_t)\right)+\nabla f(\overline{\bm{x}}_t)\right\|^2\\
\leq & \sigma^2 + 3\mathbb{E}\left\|\nabla f_i(\bm{x}_t^{(i)})-\nabla f_i(\overline{\bm{x}}_t)\right\|^2 + 3\mathbb{E}\left\|\nabla f_i(\overline{\bm{x}}_t)-\nabla f(\overline{\bm{x}}_t)\right\|^2\\
& + 3\mathbb{E}\left\|\nabla f(\overline{\bm{x}}_t)\right\|^2\\
\leq & \sigma^2+3L^2\mathbb{E}\left\|\overline{\bm{x}}_t-\bm{x}_t^{(i)}\right\|^2+3\zeta^2+3\mathbb{E}\left\|\nabla f(\overline{\bm{x}}_t)\right\|^2,
\end{align*}
which means
\begin{align*}
\mathbb{E}\left\|G(X_t,\xi_t)\right\|^2\leq &
\sum_{i=1}^{n}\left\|\nabla F_i(\bm{x}_t^{(i)};\xi_t^{(i)})\right\|^2\\
\leq & n\sigma^2+3L^2\sum_{i=1}^n\mathbb{E}\left\|\overline{\bm{x}}_t-\bm{x}_t^{(i)}\right\|^2+3n\zeta^2+3n\mathbb{E}\left\|\nabla f(\overline{\bm{x}}_t)\right\|^2\\
 = & n\sigma^2+3L^2\mathbb{E}\left\|X_t(I - A_n)\right\|^2_F+3n\zeta^2+3n\mathbb{E}\left\|\nabla f(\overline{\bm{x}}_t)\right\|^2.
\end{align*}

\end{proof}


\begin{lemma}\label{lemma:bound_pow0}
For any matrix sequence $\{M_t\}$, we have
\begin{align*}
\sum_{t=0}^{T-1}\left\| \sum_{s=0}^t M_s(I - A_n)W_{\eff}^{t-s} \right\|^2_F \leq  \frac{1}{(1-\lambda_2)^2}\sum_{t=0}^{T-1}\left\|  M_t \right\|^2_F.
\end{align*}
\end{lemma}


\begin{proof}
Since $W_{\eff}$ is symmetric, so we decompose it as
\begin{align*}
W_{\eff} = P\Lambda P^{\top} = \sum_{i=1}^n \lambda_i(W_{\eff})\bm{v}^{(i)}\left(\bm{v}^{(i)}\right)^{\top},
\end{align*}
where $\bm{v}^{(i)}$ is the corresponding eigenvector of $\lambda_i(W_{\eff})$. Meanwhile, we have 
\begin{align*}
W\frac{\bm{1}}{n} = \frac{\bm{1}}{n},
\end{align*}
 which means
 \begin{align*}
 W_{\eff} = A_n + \sum_{i=2}^n \lambda_i(W_{\eff})\bm{v}^{(i)}\left(\bm{v}^{(i)}\right)^{\top}.
 \end{align*}

Since $W_{\eff}^t = P\Lambda^t P^{\top}$, we have for any $r$ and $s$ 
\begin{align}
\left\|  M_r W_{\eff}^s-M_sA_n \right\|^2_F = &\left\|  M_r (W^s_{\eff}-A_n) \right\|^2_F \nonumber\\
= & \left\| M_r P\Lambda^sP^{\top}-M_r P\begin{pmatrix}
1,0,\cdots,0\\0,0,\cdots,0\\ \cdots \\0,0,\cdots,0
\end{pmatrix}P^{\top}\right\|^2_F \nonumber \\
= & \left\| M_r P\Lambda^s-M_r P\begin{pmatrix}
1,0,\cdots,0\\0,0,\cdots,0\\ \cdots \\0,0,\cdots,0
\end{pmatrix}\right\|^2_F \nonumber \\
= & \left\| M_r P\begin{pmatrix}
&0,&0,&0,&\cdots,&0\\
&0,&\lambda_2^s,&0,&\cdots,&0\\
&0,&0,&\lambda_3^s,&\cdots,&0\\
& \hdotsfor{5}\\
&0,&0,&0,&\cdots,&\lambda_n^s
\end{pmatrix}\right\|^2_F \nonumber\\
\leq & \left\|\lambda_2^{t}M_r P\right\|^2_F \nonumber\\
= & \left\|\lambda_2^{s}M_r \right\|^2_F. \label{eq:lemma6_1}
\end{align}

Therefore, we can have
\begin{align*}
\sum_{t=0}^{T-1} \left\| \sum_{s=0}^t M_s(I - A_n)W_{\eff}^{t-s} \right\|^2_F = & \sum_{t=0}^{T-1}\left\| \sum_{s=0}^t M_s W_{\eff}^{t-s} -M_sA_n \right\|^2_F   \\
\leq & \sum_{t=0}^{T-1}  \left ( \sum_{s=0}^t  \left\| M_s W_{\eff}^{t-s} -M_sA_n \right\|_F \right ) ^2 \\
\leq & \sum_{t=0}^{T-1}  \left ( \sum_{s=0}^t  \lambda_2^{t-s} \left \| M_s\right\|_F \right ) ^2, \quad \text{ (due to \eqref{eq:lemma6_1})} \\
\leq & \frac{1}{(1-\lambda_2)^2}\sum_{t=0}^{T-1}  \left \| M_t \right\|_F ^2, \quad \text{ (due to Lemma \ref{lemma:seq})}
\end{align*}
where the first equality holds due to $A_n W_\eff = A_n [(1-\eta)I + \eta  W] = (1-\eta ) A_n + \eta A_n = A_n$.

\end{proof}


\begin{lemma}\label{lemma:bound_diff_X}
For $\OA$, if 
\begin{align*}
(2 - \lambda_n )^2(3 - 2\lambda_n) \leq & \frac{1}{\alpha^2},\\
 1 -3C_5L^2\gamma^2 \geq & 0,
\end{align*}
we have
\begin{align*}
\sum_{t=0}^{T-1} \mathbb E\left\|X_t(I - A_n)\right\|_F^2 \leq \frac{C_5\gamma^2n\sigma^2 T}{1 -3C_5L^2\gamma^2} + \frac{3nC_5\gamma^2\zeta^2 T}{1 -3C_5L^2\gamma^2} + \sum_{t=0}^{T-1}\frac{3nC_5 \gamma^2\mathbb{E}\left\|\nabla f(\overline{\bm{x}}_t)\right\|^2}{1 -3C_5L^2\gamma^2}.
\end{align*}

\end{lemma}

\begin{proof}
From \eqref{supp:key_eq1}, we have
\begin{align*}
X_t(I - A_n) =& - \gamma \sum_{s=0}^{t-1}G_sW_{\eff}^{t-s}(I - A_n) + \sum_{s=0}^{t-2} \Delta_{s} (W_{\eff}-I)^2W_{\eff}^{t-2-s}(I - A_n) \\
&- \Delta_{t-1}(W_{\eff}-I)(I - A_n)\\
= & - \gamma \sum_{s=0}^{t-1}G_sW_{\eff}^{t-s}(I - A_n) + \sum_{s=0}^{t-2} \Delta_{s} (W_{\eff}-I)^2W_{\eff}^{t-2-s} - \Delta_{t-1}(W_{\eff}-I),
\end{align*}
so we have
\begin{align*}
\left\|X_t(I - A_n)\right\|_F^2 \leq & 3 \gamma^2 \left\|\sum_{s=0}^{t-1}G_sW_{\eff}^{t-s}(I - A_n)\right\|^2_F + 3\left\| \sum_{s=0}^{t-2} \Delta_{s} (W_{\eff}-I)^2W_{\eff}^{t-2-s} \right\|^2_F \\
&+ 3\left\| \Delta_{t-1}(W_{\eff}-I) \right\|_F^2,
\end{align*}
which leads to 
\begin{align*}
&\sum_{t=0}^{T-1} \mathbb E\left\|X_t(I - A_n)\right\|_F^2\\
 \leq & 3 \gamma^2\sum_{t=0}^{T-1} \mathbb E \left\|\sum_{s=0}^{t-1}G_sW_{\eff}^{t-s}(I - A_n)\right\|^2_F + 3\sum_{t=0}^{T-1} \mathbb E\left\| \sum_{s=0}^{t-2} \Delta_{s} (W_{\eff}-I)^2W_{\eff}^{t-2-s} \right\|^2_F\\
 & + 3\sum_{t=0}^{T-1} \mathbb E\left\| \Delta_{t-1}(W_{\eff}-I) \right\|_F^2.\numberthis\label{lemma:bound_diff_eq1}
\end{align*}
From Lemma(Too be added) we have
\begin{align*}
\sum_{t=0}^{T-1}\left\|\sum_{s=0}^{t-1}G_sW_{\eff}^{t-s}(I - A_n)\right\|^2_F \leq \frac{1}{(1-\lambda_2)^2}\sum_{t=0}^{T-2}\left\|G_t\right\|^2_F,\numberthis\label{lemma:bound_diff_eq1_2}
\end{align*}
using Lemma~\ref{lemma:bound_pow2}, we have
\begin{align*}
\sum_{t=0}^{T-1}\left\| \sum_{s=0}^{t-2} \Delta_{s} (W_{\eff}-I)^2W_{\eff}^{t-2-s} \right\|^2_F \leq \sum_{t=0}^{T-3} \left\|\Delta_{t}(W_{\eff}-I) \right\|_F^2.\numberthis\label{lemma:bound_diff_eq1_3}
\end{align*}
Taking \eqref{lemma:bound_diff_eq1_2} and \eqref{lemma:bound_diff_eq1_3} into \eqref{lemma:bound_diff_eq1} we get
\begin{align*}
&\sum_{t=0}^{T-1} \mathbb E\left\|X_t(I - A_n)\right\|_F^2\\
\leq & \frac{3\gamma^2}{(1-\lambda_2)^2}\sum_{t=0}^{T-2}\left\|G_t\right\|^2_F + 3\sum_{t=0}^{T-3} \left\|\Delta_{t}(W_{\eff}-I) \right\|_F^2 + 3\sum_{t=0}^{T-1} \mathbb E\left\| \Delta_{t-1}(W_{\eff}-I) \right\|_F^2\\
\leq & \frac{3\gamma^2}{(1-\lambda_2)^2}\sum_{t=0}^{T-2}\left\|G_t\right\|^2_F + 6\sum_{t=0}^{T-1} \left\|\Delta_{t}(W_{\eff}-I) \right\|_F^2.
\end{align*}
Using Lemma~\ref{lemma:bound_compress_error} to bound $\sum_{t=0}^{T-1} \left\|\Delta_{t}(W_{\eff}-I) \right\|_F^2$, then we get
\begin{align*}
\sum_{t=0}^{T-1} \mathbb E\left\|X_t(I - A_n)\right\|_F^2 \leq &\frac{3\gamma^2}{(1-\lambda_2)^2}\sum_{t=0}^{T-2}\left\|G_t\right\|^2_F + 6C_4\gamma^2\sum_{t=0}^{T-1} \left\|G_t\right\|^2_F\\
\leq & \left( \frac{3}{(1-\lambda_2)^2} + 6 C_4\right)\gamma^2\sum_{t=0}^{T-1} \left\|G_t\right\|^2_F.
\end{align*}
Using Lemma~\ref{lemma:bound_G}, the equation above becomes
\begin{align*}
& \sum_{t=0}^{T-1} \mathbb E\left\|X_t(I - A_n)\right\|_F^2 \\
\leq &\left( \frac{3\gamma^2}{(1-\lambda_2)^2} + 6 C_4\gamma^2\right) \left( n\sigma^2 T +3L^2\mathbb{E}\left\|X_t(I - A_n)\right\|^2_F T +3n\zeta^2T+3n\sum_{t=0}^{T-1}\mathbb{E}\left\|\nabla f(\overline{\bm{x}}_t)\right\|^2  \right)\\
\leq & C_5 \gamma^2 n\sigma^2T + 3C_5 \gamma^2L^2\mathbb{E}\left\|X_t(I - A_n)\right\|^2_F T+3nC_5 \gamma^2\zeta^2 T+3nC_5 \gamma^2\sum_{t=0}^{T-1}\mathbb{E}\left\|\nabla f(\overline{\bm{x}}_t)\right\|^2,
\end{align*}
which leads to 
\begin{align*}
&\left( 1 - 3C_5L^2\gamma^2  \right)\sum_{t=0}^{T-1} \mathbb E\left\|X_t(I - A_n)\right\|_F^2\\
 \leq &  \frac{C_5\gamma^2n\sigma^2 T}{1 -3C_5L^2\gamma^2} + \frac{3nC_5\gamma^2\zeta^2 T}{1 -3C_5L^2\gamma^2} + \sum_{t=0}^{T-1}\frac{3nC_5 \gamma^2\mathbb{E}\left\|\nabla f(\overline{\bm{x}}_t)\right\|^2}{1 -3C_5L^2\gamma^2}.
\end{align*}
So if $ 1 -3C_5L^2\gamma^2 \geq 0 $, then we have
\begin{align*}
\sum_{t=0}^{T-1} \mathbb E\left\|X_t(I - A_n)\right\|_F^2 \leq \frac{C_5\gamma^2n\sigma^2 T}{1 -3C_5L^2\gamma^2} + \frac{3nC_5\gamma^2\zeta^2 T}{1 -3C_5L^2\gamma^2} + \sum_{t=0}^{T-1}\frac{3nC_5 \gamma^2\mathbb{E}\left\|\nabla f(\overline{\bm{x}}_t)\right\|^2}{1 -3C_5L^2\gamma^2}.
\end{align*}



\end{proof}













%Since 
%\begin{align*}
%X_{t} = \left(X_{t-1} - \gamma G_{t-1} \right) W_{\eff} + (\Delta_{t-1} - \Delta_t ),
%\end{align*}
%So we have
%\begin{align*}
%X_{t} = & X_0W_{\eff}^t - \gamma \sum_{s=0}^{t-1}G_sW_{\eff}^{t-s} + \sum_{s=0}^{t-1} (\Delta_{s-1} - \Delta_s )W_{\eff}^{t-1-s}\\
%= &  - \gamma \sum_{s=0}^{t-1}G_sW_{\eff}^{t-s} + \sum_{s=0}^{t-1} \Delta_{s-1} W_{\eff}^{t-1-s} - \sum_{s=0}^{t-1} \Delta_{s} W_{\eff}^{t-1-s}\\
%= & - \gamma \sum_{s=0}^{t-1}G_sW_{\eff}^{t-s} + \sum_{s'=-1}^{t-2} \Delta_{s'} W_{\eff}^{t-2-s'} - \sum_{s=0}^{t-1} \Delta_{s} W_{\eff}^{t-1-s}\\
%= & - \gamma \sum_{s=0}^{t-1}G_sW_{\eff}^{t-s} + \sum_{s=0}^{t-2} \Delta_{s} W_{\eff}^{t-2-s} - \sum_{s=0}^{t-2} \Delta_{s} W_{\eff}^{t-1-s}\\
%& + \Delta_{-1} W_{\eff}^{t-1} - \Delta_{t-1} \\
%= & - \gamma \sum_{s=0}^{t-1}G_sW_{\eff}^{t-s} + \sum_{s=0}^{t-2} \Delta_{s} (W_{\eff}-I)W_{\eff}^{t-2-s} - \Delta_{t-1}(W_{\eff}-I). \numberthis\label{supp:eq_full_expansion}
%\end{align*}
%
%
%From Assumption XXX, for $\Delta_t$, we have
%\begin{align*}
%\mathbb E\|\Delta_t\|^2_F \leq & \alpha^2 \left\|X_t - \gamma G_t + \Delta_{t-1} \right\|^2_F\\
%= & \left\|- \gamma \sum_{s=0}^{t-1}G_sW_{\eff}^{t-s} + \sum_{s=0}^{t-2} \Delta_{s} (W_{\eff}-I)W_{\eff}^{t-2-s} - \Delta_{t-1} - \gamma G_t + \Delta_{t-1} \right\|^2_F\\
%= &  \left\|- \gamma \sum_{s=0}^{t}G_sW_{\eff}^{t-s} + \sum_{s=0}^{t-2} \Delta_{s} (W_{\eff}-I)W_{\eff}^{t-2-s}  \right\|^2_F \\
%\leq &  (1 + \beta_1 )\left\| \sum_{s=0}^{t-2} \Delta_{s} (W_{\eff}-I)W_{\eff}^{t-2-s}  \right\|^2_F + \left(1 + \frac{1}{\beta_1} \right)\left\|- \gamma \sum_{s=0}^{t}G_sW_{\eff}^{t-s}   \right\|^2_F
%\end{align*}


\section*{Proof of Theorem~\ref{theo} }
Recall that the updating rule of $\OA$ can be written in an equivalent form as follows
\begin{align*}
\Delta_t =& (X_t - \gamma G_t) + \Delta_{t-1} - C_{\omega}\left[ (X_t - \gamma G_t) + \Delta_{t-1} \right]\\
X_{t+1} =& (X_t - \gamma G_t) W_{\eff}+ \eta (\Delta_{t-1} - \Delta_t) (W_{\eff}-I)
\end{align*}
where 
\begin{align*}
W_{\eff} := (1-\eta)I + \eta W.
\end{align*}
Below we assume that $\eta\leq \frac{1}{2}$, so that $W_{\eff}\succeq 0$.

Our proof of Theorem \ref{theo} is mainly based on Lemma \ref{lemma:key_theo_lemma}. We give the proof of Theorem \ref{theo} as follows.

\paragraph{Proof of Theorem~\ref{theo}}
\begin{proof}
 If $\eta$ satisfies
\begin{align*}
\eta \leq & \min\left\{\frac{1}{2},\frac{\alpha^{-\frac{2}{3}} - 1}{4}\right\},
\end{align*}
and
\begin{align*}
\lambda_n = (1-\eta ) + \eta\lambda_n(W) > 1 - \eta - \eta = 1-2\eta,
\end{align*}
we have
\begin{align*}
(2 - \lambda_n )^2(3 - 2\lambda_n) < (1 + 2\eta)^2(1 + 4\eta)\leq (1 + 4\eta)^3\leq \frac{1}{\alpha^2}.
\end{align*}
So if 
\begin{align*}
(1 + 4\eta)^3 \leq & \frac{1}{\alpha^2},\quad\text{and}\quad
\eta \leq \frac{\alpha^{-\frac{2}{3}} - 1}{4}.
\end{align*}
Then we can ensure that
\begin{align*}
W_{\eff} \succeq & 0,\\
(2 - \lambda_n )^2(3 - 2\lambda_n) \leq & \frac{1}{\alpha^2}.
\end{align*}
{Then Theorem~\ref{theo} can be easily verified by replacing $\lambda_2 = 1-\eta + \eta \lambda_2(W) $ and $\lambda_n= 1-\eta + \eta \lambda_n(W) $ in Lemma~\ref{lemma:key_theo_lemma}.} 
%
%According to Lemma \ref{lemma:key_theo_lemma}, we can have
%\begin{align*}
%&\left(\frac{\gamma}{2} -\frac{3C_5L^2 \gamma^3}{2 -6C_5L^2\gamma^2} \right)\sum_{t=0}^T E \left\|\nabla f(\overline{\bm{x}}_t)\right\|^2\\
%\leq & \mathbb E f\left(\overline{\bm{x}}_{0} \right) - \mathbb E f\left(\bm{x}^* \right) - \left(\frac{\gamma}{2} -\frac{L\gamma^2}{2}   \right)\mathbb{E}\sum_{t=0}^{T-1}\left\|\nabla f(\overline{\bm{x}}_t)\right\|^2 + \left(\frac{L\gamma^2}{2} + \frac{C_5L^2\gamma^3}{2 -6C_5L^2\gamma^2)}\right)\sigma^2T + \frac{3C_5L^2\gamma^3\zeta^2T}{2 -6C_5L^2\gamma^2}.
%\end{align*}
%where we let
%\begin{align*}
%C_4 := & \frac{\alpha^2}{(1 - \alpha^2(2-\lambda_n)^2(3 -2\lambda_n) )(1-\lambda_n)^2} , \qquad  C_5 := \frac{3}{(1-\lambda_2)^2} + 6C_4,
%\end{align*}
%and $\lambda_n = \lambda_n(W_{\eff})$ and $\lambda_2 = \lambda_2(W_{\eff})$ for short.
%
%Notice that the third restriction $ 1 -3C_5L^2\gamma^2 \geq  0$ can be easily satisfied by using a small learning rate. However, we ensure the second restriction is satisfied, we must adjust the averaging rate $\eta$ so that $ (1- \lambda_n)$ is small enough.
\end{proof}




\section{Proof of Corollary \ref{coro}}
\begin{proof}
From Theorem\ref{theo}, we have
\begin{align*}
&\left(\frac{\gamma}{2} -\frac{3C_2L^2 \gamma^3}{2 -6C_2L^2\gamma^2} \right)\sum_{t=0}^T E \left\|\nabla f(\overline{\bm{x}}_t)\right\|^2\\
\leq & \mathbb E f\left(\overline{\bm{x}}_0 \right) - \mathbb E f\left(\bm{x}^* \right)  + \left(\frac{L\gamma^2}{2n} + \frac{C_2L^2\gamma^3}{2 -6C_2L^2\gamma^2}\right)\sigma^2T + \frac{3C_2L^2\gamma^3\zeta^2T}{2 -6C_2L^2\gamma^2},
\end{align*}
which can be rewritten as
\begin{align*}
& \left(1 -\frac{3C_2L^2 \gamma^2}{1 -3C_2L^2\gamma^2} \right)\sum_{t=0}^T E \left\|\nabla f(\overline{\bm{x}}_t)\right\|^2\\
\leq & \frac{2 \mathbb E f\left(\overline{\bm{x}}_0 \right) - 2\mathbb E f\left(\bm{x}^* \right) }{\gamma}   + \left(\frac{L\gamma}{n} + \frac{C_2L^2\gamma^2}{1 -3C_2L^2\gamma^2}\right)\sigma^2T + \frac{3C_2L^2\gamma^2\zeta^2T}{1 -3C_2L^2\gamma^2}.
\end{align*}
So if 
\begin{align*}
\gamma \leq & \frac{1}{3L\sqrt{C_2}},\\
3C_2L^2\gamma^2 \leq & \frac{1}{3},
\end{align*}
we have
\begin{align*}
 1- \frac{3C_2L^2 \gamma^2}{1 -3C_2L^2\gamma^2} \leq 1 - \frac{1}{2} = \frac{1}{2}.
\end{align*}
Choosing $\gamma = \frac{1}{3L\sqrt{C_2} + \sigma\sqrt{\frac{T}{n}} + \zeta^{\frac{2}{3}}T^{\frac{1}{3}}} $, it can be easily verified that
\begin{align*}
\frac{1}{T}\sum_{t=0}^T E \left\|\nabla f(\overline{\bm{x}}_t)\right\|^2 \lesssim \left(\frac{1}{\sqrt{nT}} + \frac{C_2}{T}\right)\sigma +  
\frac{C_2\zeta^{\frac{2}{3}}}{T^{\frac{1}{3}}} + \frac{1 + \sqrt{C_2} }{T}.
\end{align*}




Since $\eta = \min\{\frac{1}{2},\frac{\alpha^{\frac{-2}{3}} - 1}{4}\} $, so we have
\begin{align*}
C_0 = & \eta(1 - \lambda_n(W))\leq  2\eta\\
C_1 = & \frac{\alpha^2}{\left(1 - \alpha^2\left(1 + C_0\right)^2(1 + 2C_0) \right)C_0^2} \leq \frac{\alpha^2}{4\left(1 - \alpha^2\left(1 + 4\eta\right)^3 \right)\eta^2}\leq \frac{\alpha^2}{2\left( \alpha^{\frac{-2}{3}} - 1 \right)},
\end{align*}
which gives us
\begin{align*}
C_2 = & \frac{3}{\eta^2(1-\lambda_2(W))^2} + 6C_1 \lesssim \frac{1}{(1 - \lambda_2(W))^2}\left ( 1+  \frac{\alpha^2}{2\left( \alpha^{\frac{-2}{3}} - 1 \right)} \right)
\end{align*}


\end{proof}

















==> exp.tex <==
\section{Experiments}

In this section, we further demonstrate the superiority of the $\OA$ algorithm through 
an empirical study. Under aggressive compression ratios, we show the epoch-wise 
convergence results of $\OA$ and compare them with centralized
SGD (AllReduce), decentralized SGD without compression (D-PSGD \citep{lian2017can}),
and other existing decentralized compression algorithms (ECP-PSGD, DCP-PSGD
\citep{NIPS2018_7992}, and Choco-SGD \citep{Koloskova:2019aa}).


\subsection{Experimental Setup}

\paragraph{Dataset} We benchmark the algorithms with a standard image
classification task: CIFAR10 using ResNet-20. This dateset has a training
set of 50,000 images and a test set of 10,000 images, where each image is given
one of the 10 labels.

\paragraph{Communication} The communication is implemented based on NVIDIA
NCCL for AllReduce and gloo for all other algorithms. The workers are connected in a ring network so that each worker has two neighbors.

\paragraph{Compression} We use bit compression for all the compression
algorithms, where every element of the tensor sent out or received by a worker
is compressed to 4 bits or 2 bits. A number representing the Euclidean norm of
the original tensor is also sent together, so that when a worker receives the
compressed tensor, it can scale it to get a tensor with the same Euclidean norm
as the uncompressed tensor.

\paragraph{Hardware} The experiments are done on 8 2080Ti GPUs, where each GPU
is treated as a single worker in the algorithm.

\subsection{Convergence Efficiency}

We compare the algorithms with 4bit and 2bit compression, and the convergence
results are shown in Figure \ref{fig:4bit}. We use a batch size of 128 and tune
the learning rate in a $\{1, 0.5, 0.1, 0.01\}$ set for each algorithm. The
learning rate is decreased by 5x every 60 epochs. 

Note that, compared with uncompressed methods, 4bit compression saves 7/8 of the communication cost 
while 2bit compression reduces the cost by 93.75\%. The results
show that under 4bit compression, $\OA$ converges similar to uncompressed
algorithms. $\OA$ is slightly better
than Choco-SGD \citep{Koloskova:2019aa}, and converges much faster than DCP-PSGD and ECD-PSGD.
Note that DCP-PSGD does not converge under 4bit compression (as stated in the
original paper \citep{NIPS2018_7992}), and ECD-PSGD does not converge under 2bit compression.
Under 2bit compression, $\OA$ converges slower than uncompressed algorithms, but is
still faster than any other compression algorithms. The reason is that the less
bits we have, the more we gain from the error compensation in $\OA$, and
consequently $\OA$ gets a faster convergence.

The experimental results further confirm that $\OA$ achieves outstanding communication cost reduction (up to 93.75\%) without much sacrifice on convergence.

\begin{figure}
  \centering
  \includegraphics[width=0.49\textwidth]{plot/4bit-train.pdf}
  \includegraphics[width=0.49\textwidth]{plot/2bit-train.pdf}
  \caption{Epoch-wise convergence for the algorithms with 8 workers connected on a ring network. 4bit compression is on the left and 2bit compression is on the right. Note that DCP-PSGD (marked
    with *) does not
    converge below 4bit compression as stated in the original paper \citep{NIPS2018_7992},
    and ECP-PSGD does not converge under 2bit compression, so they are not shown in the figure.\label{fig:4bit}}
\end{figure}

\section{Conclusion}
This paper applies the error-compensated compression strategy, which receives big successes in centralized training, to the decentralized training. Through elaborated algorithm, the proposed $\OA$ algorithms is proven to admit higher tolerance on the compression ratio than existing compression based decentralized training. Both theoretical analysis and empirical study validate our algorithm and theorem. 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

